Learning to Super-Resolve Blurry Images with Events

Super-Resolution from a single motion Blurred image (SRB) is a severely ill-posed problem due to the joint degradation of motion blurs and low spatial resolution. In this paper, we employ events to alleviate the burden of SRB and propose an Event-enhanced SRB (E-SRB) algorithm, which can generate a sequence of sharp and clear images with High Resolution (HR) from a single blurry image with Low Resolution (LR). To achieve this end, we formulate an event-enhanced degeneration model to consider the low spatial resolution, motion blurs, and event noises simultaneously. We then build an event-enhanced Sparse Learning Network (eSL-Net++) upon a dual sparse learning scheme where both events and intensity frames are modeled with sparse representations. Furthermore, we propose an event shuffle-and-merge scheme to extend the single-frame SRB to the sequence-frame SRB without any additional training process. Experimental results on synthetic and real-world datasets show that the proposed eSL-Net++ outperforms state-of-the-art methods by a large margin. Datasets, codes, and more results are available at https://github.com/ShinyWang33/eSL-Net-Plusplus.

==> realdata_image.tex <==
\def\imwidth{0.2}


\def\ssxxs{(0.28,0.78)} % 杯子 勺
\def\ssxxsr{(-0.55,-0.55)} % 杯子 垫
\def\sxxx{(-0.4,-0.8)}%窗户 线
\def\sxxxr{(0.2,0.5)}%窗户 栏

% \def\sxxxx{(0.1,1.16)}%枕头 手 绿
% \def\sxxxxr{(0.85,-0.1)}%枕头 右 红
\def\sxxxx{(-0.5,-0.6)}%she 手 绿
\def\sxxxxr{(1,0.25)}%she 右 红

\def\ssxxsl{(0.26,0.83)} % 杯子 勺 ledvdi
\def\ssxxsrl{(-0.62,-0.46)} % 杯子 垫ledvdi
\def\sxxxl{(-0.4,-0.8)}%窗户 线
\def\sxxxrl{(0.05,0.6)}%窗户 栏

% \def\sxxxxl{(0.15,1.13)}%枕头 手 绿ledvdi
% \def\sxxxxrl{(0.65,-0.25)}%枕头 右 红ledvdi
\def\sxxxxl{(-0.5,-0.6)}%she 手 绿ledvdi
\def\sxxxxrl{(0.92,0.25)}%she 右 红ledvdi

\def\ssyys{(1.8,-2.3)}
\def\ssyysr{(-0.05,-2.3)}


\def\ssyy{(-0.8,-0.85)}
\def\ssizz{1.77cm}
\def\sswidth{0.245\textwidth}
\def\ssmag{5}
\def\scc{(2.12,1.4)}
\begin{figure*}[htb]
\footnotesize
	\centering

    \subfigure{
    	\begin{minipage}[t]{\imwidth\linewidth}
    		\centering
    		%input
			\begin{tikzpicture}[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
				\node {\includegraphics[width=\linewidth]{pic/realdata9/000013_blur.png}};
				\spy on \ssxxsr in node [left] at \ssyysr;
				\spy[red] on \ssxxs in node [left,red] at \ssyys;
				\end{tikzpicture}
			Blurry Image
			
			%e2vid
			\begin{tikzpicture}[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
				\node {\includegraphics[width=\linewidth]{pic/realdata9/000013_e2vid.jpg}};
				\spy on \ssxxsr in node [left] at \ssyysr;
				\spy[red] on \ssxxs in node [left,red] at \ssyys;
				\end{tikzpicture}
			E2VID+RCAN\vspace{0.3em}
    	\end{minipage}%
    }\hspace*{-1mm}
    \subfigure{
    	\begin{minipage}[t]{\imwidth\linewidth}
    		\centering
    		\begin{tikzpicture}[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
				\node {\includegraphics[width=\linewidth]{pic/realdata9/000013_gfn.png}};
				\spy on \ssxxsrl in node [left] at \ssyysr;
				\spy[red] on \ssxxsl in node [left,red] at \ssyys;
				\end{tikzpicture}
			GFN\vspace{0.3em}
			
			\begin{tikzpicture}[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
				\node {\includegraphics[width=\linewidth]{pic/realdata9/000013_e2sri.jpg}};
				\spy on \ssxxsr in node [left] at \ssyysr;
				\spy[red] on \ssxxs in node [left,red] at \ssyys;
				\end{tikzpicture}
			E2SRI+RCAN\vspace{0.3em}
    	\end{minipage}%
    }\hspace*{-1mm}
    \subfigure{
    	\begin{minipage}[t]{\imwidth\linewidth}
    		\centering
    	    \begin{tikzpicture}[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
				\node {\includegraphics[width=\linewidth]{pic/realdata9/000013_srn.jpg}};
				\spy on \ssxxsrl in node [left] at \ssyysr;
				\spy[red] on \ssxxsl in node [left,red] at \ssyys;
				\end{tikzpicture}
			SRN+RCAN\vspace{0.3em}
			
			\begin{tikzpicture}[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
				\node {\includegraphics[width=\linewidth]{pic/realdata9/000013_ledvdi.jpg}};
				\spy on \ssxxsrl in node [left] at \ssyysr;
				\spy[red] on \ssxxsl in node [left,red] at \ssyys;
				\end{tikzpicture}
			LEDVDI+RCAN\vspace{0.3em}
    	\end{minipage}%
    }\hspace*{-1mm}
	\subfigure{
		\begin{minipage}[t]{\imwidth\linewidth}
			\centering
			\begin{tikzpicture}[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
				\node {\includegraphics[width=\linewidth]{pic/realdata9/000013_cdvd.jpg}};
				\spy on \ssxxsrl in node [left] at \ssyysr;
				\spy[red] on \ssxxsl in node [left,red] at \ssyys;
				\end{tikzpicture}
			CDVD+RCAN\vspace{0.3em}
				
			\begin{tikzpicture}[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
				\node {\includegraphics[width=\linewidth]{pic/realdata9/000013_eslnet.png}};
				\spy on \ssxxsr in node [left] at \ssyysr;
				\spy[red] on \ssxxs in node [left,red] at \ssyys;
				\end{tikzpicture}
			eSL-Net\vspace{0.3em}
			
		\end{minipage}%
	}\hspace*{-1mm}
    \subfigure{
    	\begin{minipage}[t]{\imwidth\linewidth}
    		\centering
    		\begin{tikzpicture}[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
				\node {\includegraphics[width=\linewidth]{pic/realdata9/000013_edi.jpg}};
				\spy on \ssxxsrl in node [left] at \ssyysr;
				\spy[red] on \ssxxsl in node [left,red] at \ssyys;
				\end{tikzpicture}
			EDI+RCAN\vspace{0.3em}
			
			\begin{tikzpicture}[spy using outlines={green,magnification=\ssmag,size=\ssizz},inner sep=0]
				\node {\includegraphics[width=\linewidth]{pic/realdata9/000013_eslnet++.png}};
				\spy on \ssxxsr in node [left] at \ssyysr;
				\spy[red] on \ssxxs in node [left,red] at \ssyys;
				\end{tikzpicture}
			eSL-Net++\vspace{0.3em}
    	\end{minipage}%
    }
    \centering
	\caption{Qualitative results on the RWS dataset, where our proposed eSL-Net and eSL-Net++ are compared to GFN, SRN+RCAN, CDVD+RCAN, E2SRI+RCAN, EDI+RCAN, and LEDVDI+RCAN.}
	\label{real_sr}
\end{figure*}
